Tiered Sampling: An Efficient Method for Approximate Counting Sparse Motifs in Massive Graph Streams

We introduce Tiered Sampling, a novel technique for approximate counting sparse motifs in massive graphs whose edges are observed in a stream. Our technique requires only a single pass on the data and uses a memory of fixed size $M$, which can be magnitudes smaller than the number of edges. Our methods addresses the challenging task of counting sparse motifs - sub-graph patterns that have low probability to appear in a sample of $M$ edges in the graph, which is the maximum amount of data available to the algorithms in each step. To obtain an unbiased and low variance estimate of the count we partition the available memory to tiers (layers) of reservoir samples. While the base layer is a standard reservoir sample of edges, other layers are reservoir samples of sub-structures of the desired motif. By storing more frequent sub-structures of the motif, we increase the probability of detecting an occurrence of the sparse motif we are counting, thus decreasing the variance and error of the estimate. We demonstrate the advantage of our method in the specific applications of counting sparse 4 and 5-cliques in massive graphs. We present a complete analytical analysis and extensive experimental results using both synthetic and real-world data. Our results demonstrate the advantage of our method in obtaining high-quality approximations for the number of 4 and 5-cliques for large graphs using a very limited amount of memory, significantly outperforming the single edge sample approach for counting sparse motifs in large scale graphs.

==> appsingle.tex <==
\section{Additional theoretical results for \algosingle{}}

\begin{proof}[Proof of Theorem~\ref{thm:singleunbiased}]
	T
\end{proof}

==> conclusion.tex <==
\section{Conclusions}
%In this work, we study the problem of counting sparse motif in large scale graphs streams using multi-layer (tiered) reservoir sampling. We fully analyse and demonstrate the advantage of our method in a specific application for counting number of 4-cliques in a graph using a two tier sample. Through an extensive experimental analysis we show that the proposed algorithms produce high quality and low variance approximations for the number of 4-cliques for large synthetic and real datasets with billions of edges. Finally we present another application of the two tier method for estimating the number of 5-cliques in a graphs stream, which demonstrates the generality of our approach for successfully counting sparse motifs in massive graph streams.

%Our approach relies on multilayer reservoir sampling, where the base layer is a standard reservoir of edges and other layers are reservoirs of samples of sub-structures of the desired motif. 
%Our approach focuses on the well studied model of one pass stream computing on top of which we develop new algorithms for counting the number of 4-cliques in a graph

In this work, we study the problem of counting sparse motif in large scale graphs streams
using multi-layer (tiered) reservoir sampling. 
%To this extend, we propose new and novel algorithms to tackle this problem when the memory is limited? To the best of our knowledge, we are the first to ? 
We fully analyze and demonstrate the advantage of our method in a specific application for counting number of 4-cliques in a graph using a two tier sample. Through an extensive experimental analysis, we show that the proposed algorithms produce high quality and low variance approximations for the number of 4-cliques for large synthetic and real datasets with billions of edges. 

Finally, we test our proposed method/s of the two-tier method, on counting the number of 5-cliques in a graph stream. Our results, show good approximations?. We believe this to be a successful illustration of the generalizability of our approach.
